LipNet: End-to-End Sentence-level Lipreading

Lipreading is the task of decoding text from the movement of a speaker's mouth. Traditional approaches separated the problem into two stages: designing or learning visual features, and prediction. More recent deep lipreading approaches are end-to-end trainable (Wand et al., 2016; Chung & Zisserman, 2016a). However, existing work on models trained end-to-end perform only word classification, rather than sentence-level sequence prediction. Studies have shown that human lipreading performance increases for longer words (Easton & Basala, 1982), indicating the importance of features capturing temporal context in an ambiguous communication channel. Motivated by this observation, we present LipNet, a model that maps a variable-length sequence of video frames to text, making use of spatiotemporal convolutions, a recurrent network, and the connectionist temporal classification loss, trained entirely end-to-end. To the best of our knowledge, LipNet is the first end-to-end sentence-level lipreading model that simultaneously learns spatiotemporal visual features and a sequence model. On the GRID corpus, LipNet achieves 95.2% accuracy in sentence-level, overlapped speaker split task, outperforming experienced human lipreaders and the previous 86.4% word-level state-of-the-art accuracy (Gergen et al., 2016).

==> include/brendan.tex <==
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
%\newcommand{\TODO}[1]{\textbf{\color{blue}(*)}\marginpar{\textbf{\color{blue} TODO {#1}}}}
\newcommand{\TODO}[1]{\textbf{\color{magenta}(*) TODO: {#1}}\marginpar{\textbf{\color{magenta} TODO}}}

% my old math helpers
\newcommand{\deriv}[2]{\frac{d {#1}}{d {#2}}}
\newcommand{\pderiv}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\dderiv}[2]{\dfrac{d {#1}}{d {#2}}}
\newcommand{\dpderiv}[2]{\dfrac{\partial {#1}}{\partial {#2}}}

\DeclareMathOperator\sigm{sigm}

% notation specific to backprop
\newcommand{\dvz}{\frac{\partial E}{\partial \vz}}
\newcommand{\dvx}{\frac{\partial E}{\partial \vx}}
\newcommand{\dzj}{\frac{\partial E}{\partial z_j}}
\newcommand{\dxi}{\frac{\partial E}{\partial x_i}}

\newcommand{\vfmsg}{\vz}
\newcommand{\vbmsg}{\vdelta}
\newcommand{\fmsg}{z}
\newcommand{\bmsg}{\delta}

\newcommand{\param}{\theta}
\newcommand{\vparam}{\vtheta}

\newcommand{\out}{z}
\newcommand{\vout}{\vz}
\newcommand{\inp}{x}
\newcommand{\vinp}{\vx}

\newcommand{\loss}{E}

\DeclareMathOperator{\children}{children}
\DeclareMathOperator{\parents}{parents}

\newcommand{\fgraph}{G}
\newcommand{\bgraph}{\tilde G}
%\newcommand{\fgraph}{\overrightarrow{G}}
%\newcommand{\bgraph}{\overleftarrow{G}}
%\newcommand{\fgraph}{\vec{G}}
%\newcommand{\bgraph}{\reflectbox{\ensuremath{\vec{\reflectbox{\ensuremath{G}}}}}}

\newcommand\nfromto[2]{{#1\!\to\!#2}}
\newcommand\fromto[2]{^{\nfromto{#1}{#2}}}
%\newcommand\fromto[2]{_{#1\!\to\!#2}}
%\newcommand\fromto[2]{\ensuremath{[{#1}\!\to\!{#2}]}}


\newcommand{\Data}{\mathcal{D}}


